Marginalised Gaussian Processes with Nested Sampling

Gaussian Process (GPs) models are a rich distribution over functions with inductive biases controlled by a kernel function. Learning occurs through the optimisation of kernel hyperparameters using the marginal likelihood as the objective. This classical approach known as Type-II maximum likelihood (ML-II) yields point estimates of the hyperparameters, and continues to be the default method for training GPs. However, this approach risks underestimating predictive uncertainty and is prone to overfitting especially when there are many hyperparameters. Furthermore, gradient based optimisation makes ML-II point estimates highly susceptible to the presence of local minima. This work presents an alternative learning procedure where the hyperparameters of the kernel function are marginalised using Nested Sampling (NS), a technique that is well suited to sample from complex, multi-modal distributions. We focus on regression tasks with the spectral mixture (SM) class of kernels and find that a principled approach to quantifying model uncertainty leads to substantial gains in predictive performance across a range of synthetic and benchmark data sets. In this context, nested sampling is also found to offer a speed advantage over Hamiltonian Monte Carlo (HMC), widely considered to be the gold-standard in MCMC based inference.

==> images/teximage.tex <==
\frame{\begin{picture}(100,100)
\put(25,50){\dashbox{.5}(10,10){$A$}}
\put(50,50){\dashbox{.5}(10,10){$B$}}
\end{picture}}


==> tables/nlpd.tex <==

\begin{table}[htp]
\caption{\small NLPD values for various GP methods across a range of time series tasks. } 
\centering
\label{tab:ts}
\begin{sc}
% \begin{tabular}{lrrrrrrrrr}\toprule
% Kernel &SM &SM &SM &NKN &SM &SM &SM &NKN \\\cmidrule{1-9}
% Inference &ML II &HMC &NS &ML II &ML II &HMC &NS &ML II \\\cmidrule{1-9}
% Training Data &Short &Short &Short &Short &Long &Long &Long &Long \\\midrule
% airline &\textbf{4.90} &5.07 &5.36 &4.90 &7.25 &5.83 &5.22 &5.6 \\
% births &5.34 &4.66 &4.67 &5.29 &5.17 &5.23 &4.96 &5.42 \\
% call centre &8.64 &5.70 &6.54 &8.62 &11 &7.32 &7.29 &7.76 \\
% gas production &6.15 &6.23 &5.97 &6.15 &15.2 &12.36 &11 &12.4 \\
% internet &12.52 &11.23 &11.30 &12.51 &11.3 &11.40 &13.2 &12.6 \\
% mauna &2.14 &1.06 &\textbf{0.96} &2.87 &1.5 &3.32 &1.8 &3.4 \\
% radio &10.00 &2.02 &\textbf{1.95} &2.27 &2.19 &2.12 &2.07 &4.12 \\
% solar &0.03 &-0.19 &-0.17 &0.22 &1.4 &0.82 &0.584 &2.38 \\
% sulphuric &4.36 &5.43 &\textbf{5.42} &\textbf{4.57} &5.13 &5.15 &5.11 &6.32 \\
% temperature &3.39 &2.80 &\textbf{2.65} &2.99 &2.8 &2.49 &2.52 &4.2 \\
% unemployment &8.60 &6.13 &6.31 &8.56 &12.8 &11.21 &10.6 &8.5 \\
% wages &\textbf{1.67} &1.74 &2.19 &3.44 &159 &8.71 &6.59 &4.28 \\
% wheat &5.86 &4.59 &4.97 &12.64 &8.47 &6.44 &6.58 &6.24 \\
% Mean &5.66 &\textbf{4.34} &4.47 &5.77 &18.71 &6.34 &5.96 &6.40 \\
% & &0.08 &0.06 & & & & & \\
\footnotesize
\scalebox{0.67}{
\begin{tabular}{lrlrlrlrlc}\toprule
Inference &\multicolumn{2}{c}{ML-II} & \multicolumn{2}{c}{HMC}  & \multicolumn{2}{c}{\hspace{-5mm} Nested Sampling} \hspace{-5mm} & \multicolumn{2}{c}{ML-II} \\
\midrule
Kernel & \multicolumn{2}{c}{Spectral} &  \multicolumn{2}{c}{Spectral }  & \multicolumn{2}{c}{Spectral} & \multicolumn{2}{c}{NKN} \\
\midrule
Time Series & Partial\hspace{-2.6mm}   & Full & Partial\hspace{-2.6mm}  & Full &Partial\hspace{-2.6mm}   &Full & Partial\hspace{-2.6mm}   &Full \\\midrule
airline &\textbf{4.90} &7.25 &5.07 &5.83 &5.36 & \textbf{5.22} &4.90 &5.6 \\
births &5.34 &5.17 & \textbf{4.66} &5.23 &4.67 & \textbf{4.96} &5.29 &5.42 \\
call centre &8.64 &11 & \textbf{5.70} &7.32 &6.54 & \textbf{7.29} &8.62 &7.76 \\
gas production &6.15 &15.2 &6.23 &12.4 & \textbf{5.97} & \textbf{11} &6.15 &12.4 \\
internet &12.5 & \textbf{11.3} & \textbf{11.2} &11.4 &11.3 &13.2 &12.5 &12.6 \\
mauna &2.14 & \textbf{1.5} &1.06 &3.32 &\textbf{0.96} &1.8 &2.87 &3.4 \\
radio &10.0 &2.19 &2.02 &2.12 &\textbf{1.95} & \textbf{2.07} &2.27 &4.12 \\
solar &0.03 &1.4 & \textbf{-0.19} &0.82 &-0.17 & \textbf{0.58} &0.22 &2.38 \\
sulphuric &4.36 &5.13 &5.43 &5.15 &\textbf{5.42} &5.11 &\textbf{4.57} &6.32 \\
temperature &3.39 &2.8 &2.80 & \textbf{2.49} &\textbf{2.65} &2.52 &2.99 &4.2 \\
unemployment &8.60 &12.8 & \textbf{6.13} &11.2 &6.31 &10.6 &8.56 & \textbf{8.5} \\
wages &\textbf{1.67} &159 &1.74 &8.71 &2.19 &6.59 &3.44 & \textbf{4.28} \\
wheat &5.86 &8.47 & \textbf{4.59} &6.44 &4.97 &6.58 &12.6 & \textbf{6.24} \\
\midrule
Mean &5.66      &18.7     &\textbf{4.34} &6.34 &4.47 & \textbf{5.96} &5.77 &6.40 \\
     &$\pm 0.3$ & $\pm1.2$ &$\pm0.08$ &  $\pm0.03$  &$\pm0.06$ & $\pm0.03$  & & \\
\bottomrule
\end{tabular}}
\end{sc}
% \vspace{1mm}
\end{table}


% \begin{table}[h]
% \begin{tabular}{llllll}
%       & ML-II         &  &  Nested Sampling (100) &  &  Nested Sampling (500) \\
%       & -2.736     &  & -2.742                  &  & -2.7565             \\
%       & -0.881     &  & -0.877                  &  & -0.8687             \\
%       & 0.704      &  & 0.734                    &  & 0.7422              \\
%       & 11.642     &  & 1.667                   &  & 1.6635              \\
%       & 2.740      &  & 1.626                   &  & 1.6281              \\
%       & 2.861      &  & 1.586                   &  & 1.5868              \\
%       & 0.555      &  & 0.079                   &  & 0.0842              \\
%       & 1.523      &  & 0.276                   &  & 0.1538              \\
%       & 0.942      &  & 1.405                   &  & 1.3913              \\
% Median & 1.928 &  & 0.418            &  & 0.403        \\
% Mean   & 0.942      &  & 0.734                    &  & 0.7422              \\
%       &             &  &                          &  &                    
% \end{tabular}
% \caption{A comparison of NLPD values when performing regression on random samples drawn from a spectral mixture kernel.}
% \end{table}

==> tables/nlpd_partial.tex <==

\begin{table}[htp]
\caption{\small NLPD values for various GP methods across a range of truncated time series tasks, where only the first 100 points are used for training. } 
\centering
\label{tab:ts}
\begin{sc}
\footnotesize
\scalebox{0.9}{
\begin{tabular}{lccccc}\toprule
Kernel & Spectral &  Spectral  & Spectral & NKN \\
\midrule
Inference & ML-II & HMC  &  Nested Sampling  & ML-II \\
\midrule
airline &\textbf{4.90}  &5.07 &5.36  &4.90  \\
births &5.34  & \textbf{4.66}  &4.67 &5.29  \\
call centre &8.64  & \textbf{5.70}  &6.54  &8.62  \\
gas production & 6.15  &6.23 & \textbf{5.97}  &6.15 \\
internet & 12.5  & \textbf{11.2}  &11.3 &12.5  \\
mauna &2.14  &1.06  &\textbf{0.96} &2.87  \\
radio &10.0 &2.02  &\textbf{1.95}  &2.27  \\
solar &0.03  & \textbf{-0.19}  &-0.17  &0.22 \\
sulphuric &4.36  &5.43 &\textbf{5.42} &\textbf{4.57}  \\
temperature &3.39  &2.80 &\textbf{2.65} &2.99 \\
unemployment &8.60  & \textbf{6.13}  &6.31  &8.56 \\
wages &\textbf{1.67}  &1.74  &2.19 &3.44 \\
wheat &5.86  & \textbf{4.59}  &4.97 &12.6  \\
\midrule
Mean &5.66       &\textbf{4.34}  &4.47  &5.77 \\
     &$\pm 0.3$  &$\pm0.08$  &$\pm0.06$  & \\
\bottomrule
\end{tabular}}
\end{sc}
% \vspace{1mm}
\end{table}


% \begin{table}[h]
% \begin{tabular}{llllll}
%       & ML-II         &  &  Nested Sampling (100) &  &  Nested Sampling (500) \\
%       & -2.736     &  & -2.742                  &  & -2.7565             \\
%       & -0.881     &  & -0.877                  &  & -0.8687             \\
%       & 0.704      &  & 0.734                    &  & 0.7422              \\
%       & 11.642     &  & 1.667                   &  & 1.6635              \\
%       & 2.740      &  & 1.626                   &  & 1.6281              \\
%       & 2.861      &  & 1.586                   &  & 1.5868              \\
%       & 0.555      &  & 0.079                   &  & 0.0842              \\
%       & 1.523      &  & 0.276                   &  & 0.1538              \\
%       & 0.942      &  & 1.405                   &  & 1.3913              \\
% Median & 1.928 &  & 0.418            &  & 0.403        \\
% Mean   & 0.942      &  & 0.734                    &  & 0.7422              \\
%       &             &  &                          &  &                    
% \end{tabular}
% \caption{A comparison of NLPD values when performing regression on random samples drawn from a spectral mixture kernel.}
% \end{table}

==> tables/nsampling.tex <==
\begin{table}[b]  % [!htp]
\caption{NLPD values for various configurations of the nested sampling algorithm.} \label{tab: nested_configs}
\begin{center}
\scriptsize
\scalebox{0.92}{
\label{tab:nested_configs}
\begin{sc}
\begin{tabular}{lccccc}\toprule
&Fiducial & Dense & Multi-run & Prior \\\midrule
Live points &100 &500 &100 &100 \\
Runs &1 &1 &5 &1 \\
Prior &Log &Log &Log &Uniform \\ \midrule
{airline} &5.36 &4.66 &5.36 &8.88 \\
{births} &4.67 &4.68 &4.65 &4.73 \\
{Call centre} &6.54 &6.17 &6.45 &6.46 \\
{Gas production} &5.97 &6.38 &5.92 &8.10 \\
{internet} &11.3 &11.3 &11.3 &11.4 \\
{mauna} &0.96 &1.15 &1.09 &3.73 \\
{radio} &1.95 &2.03 &1.84 &2.19 \\
{solar} &-0.17 &-0.20 &-0.19 &-0.28 \\
{sulphuric} &5.42 &5.58 &5.15 &6.07 \\
{temperature} &2.65 &2.64 &2.63 &2.94 \\
{unemployment} &6.31 &6.21 &6.31 &6.26 \\
{wages} &2.19 &2.24 &2.20 &1.97 \\
{wheat} &4.97 &5.20 &5.39 &5.42 \\ \midrule
{Mean} &4.47 &4.46 &4.47  & 5.22  \\
% {Mean} &4.47 ($\pm$ 0.03) &4.46 ($\pm$ 0.02) &4.47 ($\pm$ 0.03) &5.22 ($\pm$ 0.05) \\
     &$\pm 0.03$ & $\pm0.02$ &$\pm0.03$ &  $\pm0.05$ \\
\bottomrule
\end{tabular}
\end{sc}
}
\end{center}
\end{table}


==> tables/rbf_nlpd.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
 % Note: It may be necessary to compile the document several times to get a multi-page table to line up properly
\begin{table}[t]
\begin{tabular}{lcc}
%{@{}lrr@{}}
\toprule\\
Kernel         & \multicolumn{1}{l}{RBF}  & \multicolumn{1}{l}{RBF}  \\* \midrule
%\endfirsthead
%
%\endhead
%
\bottomrule
%\endfoot
%
%\endlastfoot
%
Inference      & \multicolumn{1}{l}{ML-II} & \multicolumn{1}{l}{NS}   \\
\midrule
airline        & \textbf{13}              & \textbf{11.1}            \\
births         & \textbf{5.27}            & \textbf{5.26}            \\
call centre    & \textbf{9.21}            & \textbf{8.67}            \\
gas production & \textbf{14.9}            & 18.8                     \\
internet       & \textbf{11.2}            & 11.4                     \\
mauna          & 2.53                     & 2.53                     \\
radio          & \textbf{2.47}            & \textbf{2.46}            \\
solar          & \textbf{1.69}            & 1.74                     \\
sulphuric      & \textbf{5.17}            & \textbf{5.16}            \\
temperature    & 2.79                     & 2.8                      \\
unemployment   & \textbf{11.9}            & \textbf{11.3}            \\
wages          & \textbf{57.1}            & \textbf{33.4}            \\
wheat          & \textbf{9.8}             & \textbf{9.73}            \\
Mean           & 11.31                    & 10.2                     \\* \bottomrule
\end{tabular}
\end{table}
